Lightweight Interactive Proving inside an Automatic Program Verifier

Among formal methods, the deductive verification approach allows establishing the strongest possible formal guarantees on critical software. The downside is the cost in terms of human effort required to design adequate formal specifications and to successfully discharge the required proof obligations. To popularize deductive verification in an industrial software development environment, it is essential to provide means to progressively transition from simple and automated approaches to deductive verification. The SPARK environment, for development of critical software written in Ada, goes towards this goal by providing automated tools for formally proving that some code fulfills the requirements expressed in Ada contracts. In a program verifier that makes use of automatic provers to discharge the proof obligations, a need for some additional user interaction with proof tasks shows up: either to help analyzing the reason of a proof failure or, ultimately, to discharge the verification conditions that are out-of-reach of state-of-the-art automatic provers. Adding interactive proof features in SPARK appears to be complicated by the fact that the proof toolchain makes use of the independent, intermediate verification tool Why3, which is generic enough to accept multiple front-ends for different input languages. This paper reports on our approach to extend Why3 with interactive proof features and also with a generic client-server infrastructure allowing integration of proof interaction into an external, front-end graphical user interface such as the one of SPARK.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{P. Masci, R. Monahan, V. Prevosto (Eds.):  Formal\\
Integrated Development Environment 2018 (F-IDE 2018).\\
EPTCS 284, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.284.1}{10.4204/EPTCS.284.1}}
\pdfoutput=1

